Joint QoS-aware and Cost-efficient Task Scheduling for Fog-Cloud Resources in a Volunteer Computing System

Volunteer computing is an Internet-based distributed computing system in which volunteers share their extra available resources to manage large-scale tasks. However, computing devices in a Volunteer Computing System (VCS) are highly dynamic and heterogeneous in terms of their processing power, monetary cost, and data transferring latency. To ensure both the high Quality of Service (QoS) and low cost for different requests, all of the available computing resources must be used efficiently. Task scheduling is an NP-hard problem that is considered one of the main critical challenges in a heterogeneous VCS. Due to this, in this paper, we design two task scheduling algorithms for VCSs, named Min-CCV and Min-V. The main goal of the proposed algorithms is jointly minimizing the computation, communication and delay violation cost for the Internet of Things (IoT) requests. Our extensive simulation results show that proposed algorithms are able to allocate tasks to volunteer fog/cloud resources more efficiently than the state-of-the-art. Specifically, our algorithms improve the deadline satisfaction task rates by around 99.5% and decrease the total cost between 15 to 53% in comparison with the genetic-based algorithm.

==> Makefile <==
###########################################################
#
# Makefile for LaTeX docs
#

TEX = paper
FIGS = 
PSFIGS = $(FIGS:.pdf=.ps)

all: pdf
ps:  $(TEX).ps
pdf: $(TEX).pdf
dvi: $(TEX).dvi

clean:
	$(RM) *.synctex.gz *.out *.aux *.log *.bbl *.blg *~ \#*\# *.toc *.idx *.eps dummy
	$(RM) $(patsubst %.tex, %.ps, $(wildcard *.tex))
	$(RM) $(patsubst %.tex, %.dvi, $(wildcard *.tex))
	$(RM) $(patsubst %.tex, %.pdf, $(wildcard *.tex))

# only need -Ppdf if using CM fonts

paper.pdf: *.tex *.bib Makefile
	pdflatex paper.tex
	bibtex paper
	pdflatex paper.tex
	pdflatex paper.tex

# This is for a tool of mine that monitors files for changes via
# inotify and then executes actions. --cpk
notif:
	notif -vv *.tex *.bib make

